On Categories of Nested Conditions

Nested conditions are used, among other things, as a graphical way to express first order formulas ruling the applicability of a graph transformation rule to a given match. In this paper, we propose (for the first time) a notion of structural morphism among nested conditions, consistent with the entailment of the corresponding formulas. This reveals a structural weakness of the existing definition of nested conditions, which we overcome by proposing a new notion of span-based nested conditions, embedding the original ones. We also introduce morphisms for the latter, showing that those form a richer structure by organising the various models in a number of categories suitably related by functors.

==> algebra.tex <==
\section{The algebra of Nested Graph Conditions}

Needed definitions:
\begin{enumerate}
  \item Monoidal signature $\Sigma = \bigcup\{_n\Sigma_m\}_{n,m \in \nat}$, arity $ar(\sigma) = n$ and coarity $coar(\sigma)=m$ iff $\sigma \in {_n\Sigma_m}$.
  \item (Finite?) Edge-labeled hypergraphs: $G =\< V,E,l:E \to \Sigma, s,t:E \to V^*\>$ with: for all $e\in E$ it holds $ar(l(e)) = |s(e)|$ and $coar(l(e)) = |t(e)|.$
  \item Category of hypergraphs and their morphisms $HGraphCat$. 
  \item Need a notation for the discrete graph (set) with $n$ nodes. For example: 
  $\ul{n} = \{1,\ldots, n\}$
  \item Discrete cospan (aka \emph{ranked hypergraph}, $n,m$-hypergraphs, $n,m$-ranked hypergraph ?): $\<l,G,r\>$, with $l:\ul{n} \to V_G$, $r:\ul{m} \to V_G$.
  \item \emph{Positions}: finite strings of positive natural numbers ($\Pos$) (including the empty $\varepsilon$, if possible concatenation is juxtaposition, $w$, $iw$, $wj$ with $w \in \Pos, i,j \in \pnat$); \emph{closed set of positions}: $W \subseteq \Pos$ such that (1) it is finite, (2) it is prefix closed: $wi \in W \Rightarrow w \in W$, (3) it is downward closed (?)  $wi \in W, i > 1 \Rightarrow w(i-1) \in W$. 
\end{enumerate}  

\note{AC: We can define conditions first, and then ranked / typed ones}

\begin{definition}[(nested) conditions]
  \note{AC: Several definitions possible.}
  \begin{enumerate}
    \item
    A \emph{(nested) condition} $C$ is a finite, non-empty, ordered\footnote{AC: we order the children of each node just to give them a name using a position, but intuitively they should form a set.} tree in the category of hypergraphs. 
    Formally, $NC = \<W, c:W \to |HGraphCat|, a:W\setminus\{\varepsilon\} \to Mor(HGraphCat)\>$, where $W$ is a closed set of positions, and for each $wi \in W$, $a(wi): c(w) \to c(wi)$ is a morphism in  $HGraphCat$. 

    Typically, we denote hypergraph $c(w)$ as $C_w$. Therefore the root of $C$ is $C_{\varepsilon}$.
    \item Recursive definiton using `conditions' and `predicates' as in the 2005 paper?
    \item Coinductive definitions as in the paper with Barbara? 
    \item An $n,m$-ranked condition $\<l,C,r\>$, is a condition $C$ equipped with morphisms $l,r$ making $\<l,C_{\varepsilon},r\>$  an $n,m$-ranked hypergraph .
  \end{enumerate}
\end{definition}

In order to equip ranked graph conditions with Peircean Bicategorical structure, we define the needed algebraic operations on them, and prove that the relevant axioms hold, up to *** (semantical equivalence?).

\begin{definition}[operations on conditions]

  \begin{itemize}
    \item The \emph{discharger} $!: 1 \to 0$ is the ranked condition 
    $$\< id_{\ul{1}}, \< \{\varepsilon\}, \varepsilon\mapsto \ul{1}, \emptyset\>, ?_{\ul{1}}:
   \ul{0} \to \ul{1}\>$$  
   \item The \emph{co-discharger} $***: 0 \to 1$ is the ranked condition 
   $$\< ?_{\ul{1}}:
   \ul{0} \to \ul{1}, \< \{\varepsilon\}, \varepsilon\mapsto \ul{1}, \emptyset\>, id_{\ul{1}}\>$$

%   \item  The \emph{duplicator} is component  $\Nabla_{RS} = \<RS [\rrel{id_{RS}} RS \lrel{ [id_{RS}, id_{RS}] }] RS + RS\>$;
% %synchronises transformations between its left and two right interfaces; 
% \item The \emph{co-duplicator} is component  $\Delta_{RS} = \<RS + RS [\rrel{ [id_{RS}, id_{RS}] } RS \lrel{id_{RS}}] RS\>$;
% % synchronises transformations between its right and two left interfaces;
% \item The \emph{discharger} is component  $!_{RS} = \<RS [\rrel{id_{RS}} RS \lrel{\emptyset}] S_\varnothing\>$;
% % allows arbitrary transformations on its left interfaces;  
% \item The \emph{co-discharger} is component $?_{RS} = \<S_\varnothing [ \rrel{\emptyset} RS \lrel{id_{RS}} ] RS\>$.
% %allows arbitrary transformations on its right interface;  
\end{itemize}
\end{definition}


==> constructions.tex <==
\section{Constructions on span-based conditions}


% \subsection{Interface enrichment: A satisfaction invariant trasformation}

\begin{itemize}
  \item Shift of span-based conditions along an arrow $\shift{c}{f}$
  \item Back-shift of condition along an arrow $\bshift{c}{f}$, performing pullbacks of interfaces. 
  \item Back-shift preserves satisfaction 
  \item Prof: shift preserves and reflects satisfaction
  \item Interface enlargement: given  branch $p$ and interface decomposition $u = k;u'$, we build branch with up-arrow $u'$ taking the pushout for the down arrow, and shiting the subconditions.
  \item Proposition: Interface enlargement preserves and reflects satisfaction.
  \item Interface reduction: take subinterface $I' \subseteq I$ and look for POC of $\subseteq ; d$. If it exists, back-shift all subconditions. 
  \item ``Perfect'' interface reduction: when $I'$ is the minimal one such that all subconditions back-shift identically. This guarantees existence of morphism from the original to the new one. 
\end{itemize}  

\subsection{Root shift}

The category of span-based conditions and their morphisms provides a framework 
where one could define several constructions on conditions, typically described using categorical construction. Some of such constructions are presented in this section, and for each of them we explore whether it preserves and/or reflects satisfaction. All along the section, ``condition'' means by default ``span-based condition'', and similar for morphisms. 

\begin{definition}[shifting a condition root along an arrow]
    Let $c = (A,p_1\ccdots p_w)$ be a condition over $A$ and $f: A \to B$ an arrow. Then $c\Rshift f$, the \emph{root-shift of $c$ along $f$}, is the condition over $B$ defined as:
    \begin{itemize}
        \item $c \Rshift f = (B, p_1\Rshift f\cdots p_w\Rshift f)$
        \item $p_i \Rshift f = (u_i;f,d_i,c_i)$ for all $1\leq i\leq w$.
     \end{itemize}
\end{definition}
%
Because there is an obvious complete morphism from $c$ to $c\Rshift f$ (with $f$ as its top arrow and identities everywhere else), it follows immediately that shifting preserves and reflects satisfaction in the following sense:
%
\begin{equation}
    \label{eq:shiftPresReflSat}
    f;g \sat c \quad \iff\quad  g \sat \shift{c}{f}
\end{equation} 
%
Because of this property, we can reformulate the satisfaction preservation (and reflection) by morphisms (\pcite{sb-morphism preserves satisfaction}) in a more compact way:
%
\begin{align}
  \mbox{if $m:b \to c$ is a morphism then } &
    c \Rshift t^m \entails c \\
  \mbox{if $m:b \to c$ is a complete morphism then } &
    c \Rshift t^m \equiv c
\end{align}
%
Furthermore, it also follows that the root right-shift preserves entailment:
%
\[ b\entails c \qquad\text{implies}\qquad b\Rshift f\entails c\Rshift f \enspace. \]
%
Note that shifting a condition only affects the upper leg of the top level spans, which are composed with $f$. A condition root can also be shifted \emph{backwards} along an arrow. In this case the interfaces of the branches are affected, by not their subconditions.  

\begin{definition}[back-shifting a condition along an arrow]
    Let $c = (B,p_1\ccdots p_w)$ be a condition over $B$ and $f: A \to B$ be an arrow. Then $c\Rbshift f$, the \emph{root back-shift of $c$ along $f$} is the condition over $A$ defined as:
    \begin{itemize}
    \item $\bshift{c}{f} = (A, p_1\Rbshift f\cdots p_w\Rbshift f)$;
    \item $p_i\Rbshift f = (u'_i,f'_i;d_i,c_i) \mbox{ where } (u'_i,f'_i) \mbox{ is a pullback of } (f,u_i)$ for all $1\leq i\leq w$.
    \item $p_i\Rbshift f = (u_i\pb f,(f\pb u_i);d_i,c_i)$ for all $1\leq i\leq w$.\todo{Using special notation for pullback arrows}
    \end{itemize}
\end{definition}
%
\fcite{Rshift} provides a visualisation of the root shift and back-shift for a single branch.

\begin{figure}
\centering
\input{figs/Rshift}
\caption{Pictorial representation of root shift and backshift for a single-branch condition $c=(A,(u,d,c'))$, for arrows $f:A\to B$ and $g:C\to A$, respectively}
\flabel{Rshift}
\end{figure}

Back-shifting a condition preserves satisfaction, but in general does not reflect it.

\begin{proposition}[back-shifting preserves satisfaction]
\dlabel{bshift_preserves_sat}
\begin{equation}
    c \entails \bshift{c}{f} \Rshift f \enspace.
\end{equation}    
\end{proposition}

\begin{proof} \emph{(sketch)} Note that back-shifting preserves the conditions of the branches of $c$. Then the witness for $g \sat c$ is also a witness for $f;g \sat \bshift{c}{f}$. The resulting diagram is easily shown to commute because a pullback commutes.\qed
\end{proof}
%
In general the converse implication does not hold.\todo{AC: example where $A = \varnothing$. Then $\bshift{c}{f}$ quantifies existentially all free variables of $c$} However, there are some cases where it does.

\begin{align}
  \label{eq:bshiftPresSat}
  \mbox{if $f'_i$ is epi for each $(u'_i,f'_i;d_i,c_i)$ in $\bshift{c}{f}$ then } &
    \bshift{c}{f} \Rshift f \entails c \\
  \mbox{if $f\pb u_i$ is epi for each $1\leq i\leq |c|$ then } &
    \bshift{c}{f} \Rshift f \entails c \\
  \mbox{if $f;e=\id$ for some $e$ then } &
    \bshift{c}{f} \Rshift f \entails c
\end{align}
%
In categories like \cat{Set}, \cat{Graph} and presheaf toposes in general, where pullbacks are constructed pointwise, it is sufficient that $f$ is epi to ensure \eqref{eq:bshiftPresSat}.

First shifting forward and then back gives rise to an equivalent (though not identical) condition:
%
\begin{equation}
\eqlabel{Rshift-Rbshift}
(c\Rshift f)\Rbshift f \equiv c \enspace.
\end{equation}
%
We defer the proof because this will turn out to be a consequence of a more precise characterisation of $(c\Rshift f)\Rbshift f$, explored below (see \lref{Rshift-Rbshift-Ibshift}).

Finally, both root shift and root backward shift satisfy some natural (and expected) properties (note that these hold up to equality\footnote{more precisely, up to isomorphism} and not merely up to semantic equivalence):
%
\begin{align}
c\Rshift \id & = c \\
c\Rshift (f;g) & = c\Rshift f\Rshift g \\
c\Rbshift \id & = c \\
c\Rbshift (f;g) & = c\Rbshift g\Rbshift f
\end{align}

\subsection{Interface shift}

Rather than changing the root of a condition, we can change one of its (first-level) interfaces. Since the interfaces are branch-specific, it actually is more appropriate to define the interface shift as an operation over branches.

In this case we start with the back-shift, since for interfaces that is the easier direction.

\begin{definition}[interface back-shift]
    Let $p=(u,d,c)$ be a branch over $R$ and $f: J \to I$ an arrow. Then $p\Ibshift f$, the \emph{interface backshift of $p$ along $f$}, is defined as:
     \[ p \Ibshift f = (f;u,f;d,c) \enspace. \]
    Now let $c=(R,p_1\ccdots p_w)$ be a condition and for all $1\leq i\leq w$ let $f_i:J_i\to I_i$ be an arrow. Then $c\Ibshift (f_1\ccdots f_w)$, the \emph{interface backshift of $c$}, is defined as:
	\[ c \Ibshift (e_1\ccdots e_w) = (R,(p_1\Ibshift f_1)\cdots (p_w\Ibshift f_w)) \enspace. \]
\end{definition}
%
Again we state a number of preservation properties. In the remainder of this subsection, we equate a branch $p$ over $R$ with the single-branch condition $(R,p)$.
%
\begin{align}
\eqlabel{Ibshift-preserves}
p & \entails p\Ibshift f \\
\eqlabel{Ibshift-reflects}
p\Ibshift f & \entails p \qquad\text{ if $f$ is epi}
\end{align}
%
Using the interface backshift, we can also give a more precise characterisation of the root shift followed by the root backshift, as follows:
%
\begin{lemma}\llabel{Rshift-Rbshift-Ibshift}
Let $c=(A,p_1\ccdots p_w)$ be a condition and $f:A\to B$ an arrow. The following property holds:
\[ c\Rshift f\Rbshift f=c\Ibshift (e_1\ccdots e_w) \]
where $e_i$ for all $1\leq i\leq w$ is the unique arrow such that $e_i;((u_i;f)\pb f)=u$ and $e_i;(f\pb (u_i;f))=\id$.
\end{lemma}
%
Since all $e_i$ are epi (they are retractions by $e_i;(f\pb (u_i;f))=\id$), \eqcite{Ibshift-reflects} implies $c\Ibshift  (e_1\ccdots e_w)\entails c$, proving \eqcite{Rshift-Rbshift}.

\begin{definition}[interface forward shift]
    Let $p=(u,d,c)$ be a branch over $R$ and $f: I\to J$ an arrow. Then $c\Ishift f$, the (forward) \emph{interface shift of $p$ along $f$}, is the branch over $S$ (the pushout opbject of the span $(u,f)$) defined as:
     \[ p \Ishift f = (u\po f,d\po f,c\Rshift (f\po d)) \enspace. \]
    Now let $c=(R,p_1\ccdots p_w)$ be a condition and for all $1\leq i\leq w$ let $f_i:I_i\to J_i$ be an arrow. Then $c\Ishift (f_1\ccdots f_w)$, the (forward) \emph{interface shift of $c$}, is defined as:
	\[ c \Ishift (e_1\ccdots e_w) = (R,(p_1\Ishift f_1)\cdots (p_w\Ishift f_w)) \enspace. \]
\end{definition}
%
\fcite{Ishift} provides a visualisation of the interface back- and forward shift for a single branch.

\begin{figure}
\centering
\input{figs/Ishift}
\caption{Pictorial representation of interface back- and forward shift for a branch $(u,d,c)$, along arrows $f:J\to I$ and $g:I\to K$}
\flabel{Ishift}
\end{figure}
%
Interestingly, interface shift essentially does not change the semantics of a condition. This is stated by the following properties (of which \eqcite{Ishift-Rbshift} actually follows from \eqcite{Ishift} in combination with \eqcite{Rshift-Rbshift}).
%
\begin{align}
\eqlabel{Ishift}
p\Ishift f & \equiv p\Rshift (f\po u) \\
\eqlabel{Ishift-Rbshift}
p\Ishift f \Rbshift (f\po u) & \equiv p
\end{align}


==> cospan-based.tex <==
\section{Cospan conditions}

\begin{itemize}
\item Cospan conditions are arrow-based conditions in the category of cospans over some category --- for instance, $\Graph$ or $\Hyper$.

\item Over cospan conditions, epi-based morphisms seem to be quite reasonable, because (I believe) every cospan whose right leg is mono is itself epi when considered as an arrow in the cospan category. This means morphisms only cannot split variables, which seems hardly a restriction

\item Nevertheless, there are fewer (epi-based) morphisms over cospan conditions than one would wish, for the same reason as before. An example is given below.
\end{itemize}

\begin{example}\exlabel{no-cospan-morphism}
\fcite{no-cospan-morphism} shows two conditions $b,c$ such that $b\entails c$.
\begin{itemize}
\item $b$ encodes the property $\exists y\st \la(x,y) \wedge \neg \lb(x,x) \wedge \neg \exists z\sl \lc(y,z)$
\item $c$ encodes the property $\neg\lb(x,x)$.
\end{itemize}
The conditions are structurally very similar, and one would like to be able to ``explain" the entailment through the existence of a morphism from $b$ to $c$. However, such a morphism does not exist, essentially because the variable $y$, which does not occur in $c$, has to be kept around on the lower level of $b$.
\end{example}

\begin{figure}\flabel{no-cospan-morphism}
\centering
\subcaptionbox
  {Arrow-based condition in $\Graph$}
  {\input{figs/ex-no-cospan-morphism-ab}}
\subcaptionbox
  {Arrow-based condition in $\Cospan(\Graph)$}
  {}%\input{figs/ex-no-cospan-morphism-ab}}

\caption{Two arrow-based conditions with an entailment relation but no morphism}
\end{figure}


==> morphism-based.tex <==
\section{Arrow-based conditions}
 
In this section we recall the standard notion of nested condition, using a formulation that will make the connection with the variation proposed in this paper stand out. Here and in the remainder of the paper, we will mostly omit the term ``nested'' and just refer to \emph{conditions}; however, to distinguish them from our variation, we will refer to the standard notion of nested conditions as \emph{arrow-based}.

The definitions below use \emph{objects} and \emph{arrows} as building blocks. These can for now be thought of as the objects and arrows of any category $\bC$; however, our examples and intuitions will all be based on $\graph$.

For a given root object $R$, the set of arrow-based branches over $R$ is denoted $\MB{R}$, and the set of arrow-based conditions over in $R$ is denoted $\MC R$. They are inductively defined as follows:

\begin{definition}[arrow-based condition]\dlabel{mb condition}
  Given a root object $R$:
  \begin{itemize}
  \item A \emph{arrow-based condition} over $R$ is a pair $(R,\cB)$ where $\cB\subseteq \MB R$ is a finite set of arrow-based branches over $R$.
  \item A \emph{arrow-based branch} over $R$ is a pair $(r,c)$ where $r: R\func S$ is an arrow and $c\in \MC S$ is a arrow-based condition over $S$.
  \end{itemize}
\end{definition}
%
\emph{Terminology and notation:} We use $c,d$ to range over conditions and $p,q$ to range over branches. We use $R_c,\cB_c$ to refer to the root and branches of a condition $c$, and $R_p,r_p,S_p,c_p$ to refer to the root, arrow, subcondition root and subcondition of a branch $p$. We will also occasionally enumerate the elements of $\cB_c$ and directly write $c=(R_c, \setof{(r_i, c_i)}_{1\leq i\leq n})$ with $n=|\cB_c|$.
%
\begin{figure}
  \centering
  \input{figs/ab-condition}
  \caption{Pictorial representation of a arrow-based condition}
  \flabel{ab-condition}
\end{figure}

\medskip\noindent A condition expresses a property of arrows from its root to an arbitrary object. This is operationalised through the notion of \emph{satisfaction}.

\begin{definition}[satisfaction of arrow-based conditions]\dlabel{ab-satisfaction}
  Let $c$ be an ab-condition and $g:R_c\func G$ an arrow from $c$'s root to an object $G$. We say that \emph{$g$ satisfies $c$}, denoted $g\sat c$, if there is a branch $b\in \cB_c$ and an arrow $h:S_b\func G$ such that
  \begin{itemize}
  \item $g=r_b;h$
  \item $h\nsat c_b$.
  \end{itemize}
\end{definition}
%
\emph{Terminology and notation.} We call $b$ the \emph{responsible branch} and $h$ the \emph{witness} for $g\sat C$. Pictorially, $g\sat c$ with responsible branch $(r_i,c_i)$ and witness $h$ can be visualised as in \fcite{ab-satisfaction}.
%
\begin{figure}
  \centering
  \input{figs/ab-satisfaction}
  \caption{Pictorial representation of $g\sat c$}
  \flabel{ab-satisfaction}
\end{figure}

\medskip\noindent The notion of \emph{morphism} of nested conditions has not received much attention in the literature. Given the fact that an ab-condition is essentially a diagram in the category $\bC$, it is natural to imagine that a morphism from $c$ to $d$ should essentially be morphism between their diagrams, involving arrows from objects of $c$ to objects of $d$ such that the subdiagrams commute. However, since the semantics of conditions is really expressed by the notion of satisfaction, we want this to be preserved by morphisms, in some precise sense. For that to be the case, we need a more refined notion of morphism that plays well with the second clause of \dref{ab-satisfaction} in which there is a negation.

\begin{definition}[arrow-based condition morphism]\dlabel{ab-morphism}
  Given two ab-conditions $c,d$, an ab-condition morphism $m$ from $c$ to $d$ is a pair $(t:R_c\func R_d,\setof{m_p}_{p\in \cB_c})$ such that for all branches $p\in \cB_c$ there is a branch $q\in \cB_d$ with:
  \begin{enumerate}
  \item $m_p$ an (ab-condition) morphism from $c_q$ to $c_p$;
  \item $t;r_q;t_{m_p}=r_p$.
  \end{enumerate}
\end{definition}
%
Hence, a morphism consists of a \emph{top} arrow $t$ from the root of the source condition to that of the target condition, and for each branch $p$ of the source condition a \emph{backward} morphism $m_p$ from some branch $q$ of the target condition. We sometimes call $q$ the \emph{source branch} of $m_p$. Pictorially, $m$ can be visualised as in \fcite{ab-morphism}.
%
\begin{figure}
  \centering
  \input{figs/ab-morphism}
  \caption{Pictorial representation of a arrow-based condition morphism $m:c\func d$}
  \flabel{ab-morphism}
\end{figure}

\medskip\noindent Morphisms have the expected properties: identities and composition exist and form a monoid.
%
\begin{definition}[arrow-based composition identity]\dlabel{ab-identity}
  Given a ab-condition $c=(R,\cB)$, the identity $\id_c:c\func c$ is defined as $(\id_R,\setof{\id_{m_b}}_{b\in \cB})$.
\end{definition}

\begin{definition}[arrow-based condition morphism composition]\dlabel{ab-composition}
Given two ab-condition morphisms $m:c\func d$ and $n:d\func e$, their composition is defined as $m;n=(t_m;t_n,\setof{n_{q_p};m_p}_{p\in \cB_c})$ where for each $p\in \cB_c$, $q_p\in \cB_d$ is the source branch of $m_p$.
\end{definition}

\begin{proposition}
  Composition of arrow-based condition morphisms satisfies $\id_c;m=m=m;\id_d$ for $m:c\func d$ and $m_1;(m_2;m_3)=(m_1;m_2);m_3$ for $m_i:c_i\func c_{i+1}$ ($i=1,2,3$).
\end{proposition}



==> outline.tex <==
\section{Outline}

\begin{enumerate}
\item  Nested conditions as tree of morphisms - Satisfaction 
\item  Nested condition as tree of cospans - Satisfaction
\item \emph{Question: what's the relation with instantiation of Barbara's definition to Cospan(Graph) and the corresponding notion of satisfaction?}
\item  Translating cospan-based conditions to standard ones [easy: take all pushouts and link them]
\item  Translating standard conditions to cospan-based ones [inductive bottom-up contstruction; at each step needs to compute a unique interface taking the union]
\item Translation preserves Satisfaction
\item  Morphisms of cospan-based conditions
\item  Morphisms reflect Satisfaction
\item Algebra of nested conditions: we sketched it for the standard ones, how does it work for cospan-based ones?
\item The category of ranked cospan conditions is a FOL(?)-bicategory - morphisms among conditions with the same rank should be consistent with entailment.
\end{enumerate}

